Data-Driven Protection Levels for Camera and 3D Map-based Safe Urban Localization

Reliably assessing the error in an estimated vehicle position is integral for ensuring the vehicle's safety in urban environments. Many existing approaches use GNSS measurements to characterize protection levels (PLs) as probabilistic upper bounds on the position error. However, GNSS signals might be reflected or blocked in urban environments, and thus additional sensor modalities need to be considered to determine PLs. In this paper, we propose a novel approach for computing PLs by matching camera image measurements to a LiDAR-based 3D map of the environment. We specify a Gaussian mixture model probability distribution of position error using deep neural network-based data-driven models and statistical outlier weighting techniques. From the probability distribution, we compute the PLs by evaluating the position error bound using numerical line-search methods. Through experimental validation with real-world data, we demonstrate that the PLs computed from our method are reliable bounds on the position error in urban environments.

==> biography.tex <==
%auto-ignore
\section*{Biography}

% Biographies are defined as follows:
% \biography{Author name}{author biography text}

\biography{Shubh Gupta}{is a graduate student in the Department of Electrical Engineering at Stanford University. He received his B.Tech degree in Electrical Engineering with a minor in Computer Science and Engineering from the Indian Institute of Technology Kanpur in 2018.}

\biography{Grace X. Gao}{is an assistant professor in the Department of Aeronautics and Astronautics at Stanford University. Before joining Stanford University, she was an assistant professor at University of Illinois at Urbana-Champaign. She obtained her Ph.D. degree at Stanford University. Her research is on robust and secure positioning, navigation and timing with applications to manned and unmanned aerial vehicles, robotics and power systems.}


==> proj_err.tex <==
%auto-ignore
\subsection{Projection of Position Errors in Error Direction}
We robustly estimate the horizontal direction of position error using the $x$ and $y$-dimension position error samples and weights. For vertical dimension errors, the analogous direction is the $z$-axis itself. For brevity, we represent the outlier weights $W^{N_C}_{x, t}, W^{N_C}_{y, t}, W^{N_C}_{z, t}$, position errors $E^{N_C}_{x, t}, E^{N_C}_{y, t}, E^{N_C}_{z, t}$ and associated variances $V^{N_C}_{x, t}, V^{N_C}_{y, t}, V^{N_C}_{z, t}$ as $N_C \times 1$ matrices,
\begin{align*}
	W^{N_C}_{X, t} &= [\begin{matrix}w^{(1)}_{X, t} & \ldots & w^{(N_C)}_{X, t}\end{matrix}]^\top \\
	E^{N_C}_{X, t} &= [\begin{matrix}\Delta X_t^{(1)} & \ldots & \Delta X_t^{(N_C)}\end{matrix}]^\top \\
	V^{N_C}_{X, t} &= [\begin{matrix} (\sigma^2_{X, t})^1 & \ldots & (\sigma^2_{X, t})^{N_C}\end{matrix}]^\top,
\end{align*}
where $X=x,y,$ or $z$ dimension. Using the outlier weights $W^{N_C}_{x, t}, W^{N_C}_{y, t}$ and position errors $E^{N_C}_{x, t}, E^{N_C}_{y, t}$, we compute the horizontal error direction $\theta_{h}$,
\begin{equation}
	\theta_{h} = \atan2\left(\left(W^{N_C}_{y, t}\right)^\top \negthickspace E^{N_C}_{y, t}, \  \left(W^{N_C}_{x, t}\right)^\top \negthickspace E^{N_C}_{x, t} \right).
\end{equation}
Then, we project the position errors and variances in $x$ and $y$ dimensions to the horizontal error direction $\theta_h$ and compute the magnitudes,
\begin{align*}
	E^{2N_C}_{h, t} &= \left[\begin{matrix}
		\left|(\cos{\theta_h})^{-1} \cdot \left(E^{N_C}_{x, t}\right)^\top\right| & \left|(\sin{\theta_h})^{-1} \cdot \left(E^{N_C}_{y, t}\right)^\top\right|
	\end{matrix}\right]^\top \\
	V^{2N_C}_{h, t} &= \left[\begin{matrix}
		\left|(\cos{\theta_h})^{-2} \cdot \left(V^{N_C}_{x, t}\right)^\top\right| & \left|(\sin{\theta_h})^{-2} \cdot \left(V^{N_C}_{y, t}\right)^\top\right|
	\end{matrix}\right]^\top, 
\end{align*}
where
\begin{enumerate}
	\item[--] $E^{2N_C}_{h, t}$ denotes the $2N_C \times 1$ matrix of horizontal position error magnitudes with elements denoted as $\Delta h_t^{(i)}$
	\item[--] $V^{2N_C}_{h, t}$ denotes the $2N_C \times 1$ matrix of horizontal position error variances with elements denoted as $(\sigma^2_{h, t})^{(i)}$
	\item[--] $|\cdot|$ denotes elementwise magnitude. 
\end{enumerate}
The corresponding outlier weights $w_{h, t}^{(i)} \in W^{2N_C}_{h, t}$ are computed from $W^{N_C}_{x, t}, W^{N_C}_{y, t}$ by normalizing them to have unity sum,
\begin{equation}
	W^{2N_C}_{h, t} = \left[\begin{matrix}
		0.5 \cdot \left(W^{N_C}_{x, t}\right)^\top & 0.5 \cdot \left(W^{N_C}_{y, t}\right)^\top
	\end{matrix}\right]^\top.
\end{equation} 
Here, we simplify the problem and assume that the DNN outputs in the $x$ and $y$ dimensions are independently estimated. This assumption might not necessarily hold, since a common set of features is used in the DNN to determine the position error in all dimensions. However, we reason that the DNN loss function $\mathcal{L}(\Delta \*x^*, \Delta \*x, \log \$*\sigma^2)$ treats the position error in each of the dimensions independently, and hence the assumption of position error independence across dimensions is justified.

Since the vertical error direction is the $z$-axis itself, we simply obtain the vertical position error magnitudes $\Delta v_t^{(i)} \in E^{N_C}_{v, t}$, variances $(\sigma^2_{v, t})^{(i)} \in V^{N_C}_{v, t}$ and outlier weights $w_{v, t}^{(i)} \in W^{N_C}_{v, t}$,
\begin{align*}
	E^{N_C}_{v, t} &= |E^{N_C}_{z, t}| \\
	V^{N_C}_{v, t} &= V^{N_C}_{z, t} \\
	W^{N_C}_{v, t} &= W^{N_C}_{z, t}.
\end{align*}   

Note that the horizontal position error magnitudes $E^{2N_C}_{h, t}$ have twice the number of elements as compared with vertical error magnitudes $E^{N_C}_{v, t}$, since the horizontal errors incorporate both $x$ and $y$ dimension outputs from the DNN.

==> train_proc.tex <==
%auto-ignore
\subsection{Training Procedure}
 
We train the DNN using stochastic gradient descent. Directly optimizing via the maximum likelihood loss term $\mathcal{L}_{\textrm{MLE}}(\cdot)$ might suffer from instability caused by the interdependence between the translation error $\Delta \tilde{\*x}$ and covariance $\tilde{\Sigma}$ outputs~\cite{skafte_reliable_2019}. Therefore, we employ the mean-variance split training strategy proposed in~\cite{skafte_reliable_2019}: First, we set $(\alpha_{\textrm{Huber}}=1, \alpha_{\textrm{MLE}}=1, \alpha_{\textrm{Ang}}=1)$ and only optimize the parameters of CMRNet till validation error stops decreasing. Next, we set $(\alpha_{\textrm{Huber}}=0, \alpha_{\textrm{MLE}}=1, \alpha_{\textrm{Ang}}=0)$ and optimize the parameters of CovarianceNet. We alternate between these two steps till validation loss stops decreasing. Our DNN is implemented using the PyTorch library~\cite{paszke_pytorch_2019} and takes advantage of the open-source implementation available for CMRNet~\cite{cattaneo_cmrnet_2019} as well as the available pretrained weights for initialization. Similar to CMRNet, all the layers in our DNN use the leaky RELU activation function with a negative slope of $0.1$. We train the DNN on using a single NVIDIA Tesla P40 GPU with a batch size of $24$ and learning rate of $10^{-5}$ selected via grid search.
